Wait to be Faster: a Smart Pooling Framework for Dynamic Ridesharing

Ridesharing services, such as Uber or Didi, have attracted considerable attention in recent years due to their positive impact on environmental protection and the economy. Existing studies require quick responses to orders, which lack the flexibility to accommodate longer wait times for better grouping opportunities. In this paper, we address a NP-hard ridesharing problem, called Minimal Extra Time RideSharing (METRS), which balances waiting time and group quality (i.e., detour time) to improve riders' satisfaction. To tackle this problem, we propose a novel approach called WATTER (WAit To be fasTER), which leverages an order pooling management algorithm allowing orders to wait until they can be matched with suitable groups. The key challenge is to customize the extra time threshold for each order by reducing the original optimization objective into a convex function of threshold, thus offering a theoretical guarantee to be optimized efficiently. We model the dispatch process using a Markov Decision Process (MDP) with a carefully designed value function to learn the threshold. Through extensive experiments on three real datasets, we demonstrate the efficiency and effectiveness of our proposed approaches.

==> ack.tex <==
\section{acknowledgment}
\label{sec:ack}

If you think that this template helped you on writing research papers and you work on the related topics, please help to cite some of my publications 
\cite{cheng2016task, cheng2017utility, chen2014gmission, cheng2015reliable,  cheng2017prediction, chen2018effective, cheng2018experimental, cheng2018frog, cheng2019cooperation, chen2019minimize}. Thanks a lot!
